Winterface: An Interface from Wannier90 to Quantum Transport

In this work a framework for quantum transport simulation from first principles is introduced, focusing on the coherent case. The model is based on the non-equilibrium Green's function (NEGF) formalism and maximally localized Wannier functions (MLWFs). Any device simulation, here based on two-dimensional (2-D) materials, starts by identifying a representative unit cell, computing its electronic structure with density functional theory (DFT), and converting the plane-wave results into a set of MLWFs. From this localized representation of the original unit cell, the device Hamiltonian can be constructed with the help of properly designed upscaling techniques. Here, a powerful tool called Winterface is presented to automatize the whole process and interface the initial MLWF representation with a quantum transport solver. Its concepts, algorithms, and general functionality are discussed on the basis of a molybdenum disulfide (2-D) monolayer structure, as well as its combination with tungsten disulfide. The developed approach can be considered as completely general, restricted only by the capability of the user to perform the required DFT calculations and to "wannierize" its plane-wave results.

==> code.tex <==
\chapter{Structure of the Code}\label{chap:code}

The Winterface code is divided into two libraries \emph{libmat}, a matrix library, and \emph{liblat}, a library using libmat as its base and providing all algorithms described in the previous sections.

\section{Libmat}
\label{sec:libmat}

The libmat library started out as a wrapper for calls to BLAS functions to make the code more readable. It then grew into a more versatile framework that contains all basic functions to operate on matrices used in \emph{liblat}. The functionality of the library will not be discussed in detail, only the basics will be introduced to make the code in \emph{liblat} comprehensible. \\

Two basic design choices follow from the use of algorithms dealing with crystal lattices. Matrices often play the role of containers for vectors such as the three basis vectors describing the translational symmetry of a lattice or the positions of atoms. Such matrices can be designed to work as an array of columns, imitating the general interface of C++ standard library containers, e.g. \emph{std::vector}. In practice, this means that a special kind of iterator pointing to entire columns of a matrix spawned by the methods \emph{cBegin()} and \emph{cEnd()} must be available, as well as a variable size, where the number of rows must be specified upon creation. It is important that requesting additional space for more columns is possible at any time. Columns can then be appended using the familiar \emph{push\_back} operator. A typical piece of code looks like this:

\begin{lstlisting}
 const int M=3, N=10;
 
 // create matrix of size MxN of random numbers
 fMat mat1 = rand(M,N);
 
 // create empty matrix of size Mx0, reserve for 2N columns
 fMat mat2(M,0); mat2.reserve(2*N);
 
 // copy mat1 into mat2 column by column
 for (auto i=mat1.ccBegin(); i!=mat1.ccEnd(); ++i)
    mat2.push_back(*i);
    
 // append mat1 to mat2 in one call
 mat2.push_back(mat1);
 
 // the result is thus mat2 = [mat1 mat1]
\end{lstlisting}

This use of iterators over columns in loops is typical in \emph{liblat}. Even though working over columns is to be preferred whenever possible due to the column-major arrangement of the physical memory of CPUs, iterators over rows are provided as well. A clever use of all these iterators in conjunction with calls to the standard library of C++ is demonstrated in the next example:

\begin{lstlisting}
 const int M=8, N=12;
 fMat mat1 = rand(M,N), mat2(N,M);
 
 // write the transpose of mat1 into mat2
 std::transform(mat1.ccBegin(),mat1.ccEnd(),mat2.rBegin());
 
 // sort the columns of mat1 and the rows of mat2
 std::sort(mat1.cBegin(),mat1.cEnd(),vcmp);
 std::sort(mat2.rBegin(),mat2.rEnd(),vcmp);
\end{lstlisting}

Here,  vcmp is a lambda implementation of the relation in Eq. \eqref{sec:hctor:eq3}.\\
The second major design choice is the seamless implementation of comparators with a given tolerance level, elementwise and otherwise. This stems from the fact that matrices are used in a variety of algorithms operating on lattices where we have to consider the periodicity of the system and be especially careful with respect to finite input precision. Rounding errors can always happen due to the convention that atomic positions, in the coordinates of the translational symmetry, must always lie within the interval $[0,1)$. Practically this means that we need a tolerance level $\epsilon$ such that $[0,1)$ effectively becomes $[-\epsilon,1-\epsilon)$. Otherwise, any small error for a vector put at the origin, which is a frequent occurrence in the usual choice of atomic positions, could lead to coordinates slightly slipping into the negative. If periodicity is then enforced by applying modulus 1 on it, a correct coordinate at $-\delta$ with $0<\delta<\epsilon$ would be forced to the other side of the unit cell by resulting in $1-\delta$. In many functions, it is imperative that such translations are prevented, but when working with lattices, it is in general desirable when the positions do not appear to be jumping back and forth for no reason. In the library this is realized with the help of a tolerance level adjustable by the user and implemented as a stack of floating point numbers. At any given point in time the top of the stack is used as the current tolerance level. Consider the following example:

\begin{lstlisting}
 fMat my_func(const fMat& mat1, const fMat2& mat2) noexcept {
    // push 1e5 onto the stack, compare then pop and return
    set_mtol(1e-5);
    fMat res = mat1<mat2;
    reset_mtol();
    
    return res;
 }
 
 int main() {
    // push 1e-3 onto the stack
    set_mtol(1e-3);
    fMat mat1 = rand(3,3), mat2 = rand(3,3);
    
    // print a comparison using 1e3 first, then 1e5 inside my_func
    std::cout << "\n" << (mat1<mat2) << my_func(mat1,mat2) << "\n";
    // the level outside my_func will not notice the change inside
    
    return 0;
 }
\end{lstlisting}

In this way different tolerance levels can be used in different parts of the code. The upside is that the handling of the tolerance level is seamlessly taken care of in the background, allowing for a clean and readable code. The downside is that function calls can mess up the tolerance stack by forgetting to reset it at the end. Hence, bugs in one part of the code can be caused by other, unrelated code segments. This feature must therefore be used with great caution, especially when exceptions are thrown so that the concerned function may be closed without resetting the tolerance level. It is best practice to set and reset the tolerance explicitly around the sections where an adjustment is needed. \\
Besides the actual matrix class, a number of additional functions are provided such as the \emph{rand} function used in the examples above, as well as functions to calculate eigenvalues. A list of the available functions can be found in the file \emph{lm\_fn.h}.







\section{Liblat}
\label{sec:liblat}

This is the library that contains all of the functionality described in Chapter \ref{chap:wbh} and \ref{chap:hctor}. It can be either directly linked to OMEN or alternatively compiled as a standalone executable \emph{ltool} which offers the possibility to calculate bandstructures or to deal with lattices. The concepts discussed in Section \ref{sec:approx} are available in \emph{ltool} as well. \\

The code is subdivided into two namespaces:

\begin{itemize}
 \item \textbf{aux}: for a number of auxiliary functions and classes that are needed, but do not belong to the core library functionality.
 \item \textbf{ll\_\_}: for the core functionality. All classes have a prefix ll\_ in order to avoid naming conflicts.
\end{itemize}

The most important components of these namespaces can be visualized in Fig. \ref{sec:code:fig1} and are listed below:

\begin{figure}
 \centering
 \includegraphics[width=0.65\textwidth]{liblat}
 \caption{General organization and code structure of liblat. Boxes designate classes, bubbles collections of functions, solid arrows inheritance, while dashed arrows indicate dependencies. The central cluster of functions, \emph{ll\_omen} connects everything together. Liblat generates the Hamiltonians along bonds, calls the bandstructure tests, and prepares the input files for OMEN.}\label{sec:code:fig1}
\end{figure}

\begin{itemize}
 \item \textbf{aux\_parser}: class providing the basic functionality for reading member variables from a text file. By inheriting directly or indirectly from this class, member variables can be initialized by user inputs defined in a text file. A complex inheritance structure is possible, allowing user inputs to be split among multiple classes, whilst using the same text file as a central input.
 \item \textbf{ll\_BStest\_input}: input parameters for the bandstructure test.
 \item \textbf{ll\_wmatching\_input}: input parameters for the matching of Wannier centers to atomic positions.
 \item \textbf{ll\_omen\_input}: class combining parameters specific to the OMEN interface as well as those required for the matching process and the bandstructure test. It relies on the inheritance from the respective classes.
 \item \textbf{ll\_BStest}: bandstructure test using a mesh or a trace in k-space.
 \item \textbf{ll\_mesh}: class implementing a mesh in N-dimensional space. It is capable of conveniently generating meshes compatible with the result of the MATLAB function \emph{meshgrid} \cite{matlab_meshgrid}, but has a more generic design.
 \item \textbf{ll\_cell}: class constructing a unit cell from an atomic lattice, as introduced in Section \ref{sec:lattice}.
 \item \textbf{ll\_bonds}: class used to describe bonds in a lattice, as introduced in Section \ref{sec:wbh}.
 \item \textbf{ll\_hbonds}: specialized version of ll\_bonds including interaction data along bonds generated from Wannier90 output, as introduced in Section \ref{sec:wbh}.
 \item \textbf{ll\_hbondss}: class handling multiple instances of \emph{ll\_hbonds} based on an analogous interface. Its working principle was introduced in Section \ref{sec:approx}.
 \item \textbf{ll\_fn}: collection of utility functions used all over the code. The most important ones are:
 \begin{itemize}
  \item \emph{dist}: functions to measure distances in periodic space.
  \item \emph{genHam}: functions to generate sets of $\{ \mathbf{R},\mathcal{H}(\mathbf{R}) \}$ from Wannier Bonds Hamiltonians in supercells, to be used, for example in, bandstructure calculations.
  \item \emph{calcBS, calcFoldedBS, ...}: functions to calculate bandstructures.
 \end{itemize}
 \item \textbf{ll\_io}: functions to read data from Wannier90, VASP or OMEN outputs. Among them,  \emph{writeHamBlock}, is the basic function to create Hamiltonian matrices for any lattice compatible with the Wannier Bonds Hamiltonian data used in the process.
 \item \textbf{ll\_omen}: central cluster of functions, where OMEN's inputs are generated.
\end{itemize}

As already mentioned, the outputs of Winterface can also be transferred to other quantum transport simulators, requiring only slight modifications of the code outputs to match the format of the alternate QT tool inputs. The code was specifically designed to allow for straightforward extensions to different formats.


\clearpage

